Playing Games in the Baire Space

We solve a generalized version of Church's Synthesis Problem where a play is given by a sequence of natural numbers rather than a sequence of bits; so a play is an element of the Baire space rather than of the Cantor space. Two players Input and Output choose natural numbers in alternation to generate a play. We present a natural model of automata ("N-memory automata") equipped with the parity acceptance condition, and we introduce also the corresponding model of "N-memory transducers". We show that solvability of games specified by N-memory automata (i.e., existence of a winning strategy for player Output) is decidable, and that in this case an N-memory transducer can be constructed that implements a winning strategy for player Output.

==> eptcsdata.tex <==
\providecommand{\firstpage}{13}
\providecommand{\publicationstatus}{T. Brihaye, B. Delahaye, L. Jezequel, N. Markey, J. Srba (Eds.):\\
Cassting Workshop on Games for the Synthesis of Complex Systems\\
and 3rd International Workshop on Synthesis of Complex Parameters\\ 
(Cassting'16/SynCoP'16).\\
EPTCS 220, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.220.2}{10.4204/EPTCS.220.2}}

